Axially-deformed solution of the Skyrme-Hartree-Fock-Bogoliubov equations using the transformed harmonic oscillator basis (IV) hfbtho (v4.0): A new version of the program

We describe the new version 4.0 of the code hfbtho that solves the nuclear Hartree-Fock-Bogoliubov problem by using the deformed harmonic oscillator basis in cylindrical coordinates. In the new version, we have implemented the restoration of rotational, particle number, and reflection symmetry. The restoration of rotational symmetry does not require using bases closed under rotation. Furthermore, the SeaLL1 functional was added and the calculation of the Coulomb potential was improved. Finally, the code has been refactored to facilitate maintenance and future developments.

==> new_commands.tex <==
%
%  HFBTHO VERSION NUMBER
%
\newcommand{\codeversion}{4.0}
\newcommand{\hfbtho}{{\sc hfbtho}}
\newcommand{\hfodd}{{\sc hfodd}}
\newcommand{\hfbrad}{{\sc hfbrad}}
\newcommand{\di}{i}


%
%  PAGE CUSTOMIZATION
%
\definecolor{db}{rgb}{0.180,0.543,0.340}

\setlength{\textheight}{23cm}
\setlength{\textwidth}{17.15cm}
\setlength{\oddsidemargin}{-0.5cm}
\setlength{\evensidemargin}{-0.5cm}
\setlength{\marginparwidth}{0cm}
\setlength{\marginparsep}{0cm}
\setlength{\topmargin}{0cm}
\setlength{\headheight}{0cm}
\setlength{\headsep}{0cm}

%
%  NEW COMMANDS AND COUNTERS
%

\newcounter{mysubsubsection}
\setcounter{topnumber}{20}
\setcounter{bottomnumber}{20}
\setcounter{totalnumber}{20}
\newcounter{leteq}
\newcommand{\steplet}{\stepcounter{leteq}\addtocounter{equation}{-1}}
\newcommand{\dps}{\displaystyle}

\newcommand{\hodd}{\bf\color{red}}
\newcommand{\htho}{\bf\color{blue}}
\newcommand{\spc}{{\ }}
\newcommand{\pr}[1]{{\sc{\lowercase{#1}}}}

\newcommand{\nn}{\boldsymbol{n}}
\newcommand{\mm}{\boldsymbol{m}}
\newcommand{\nnp}{\boldsymbol{n}'}
\newcommand{\mmp}{\boldsymbol{m}'}

\newcommand{\avec}{\boldsymbol{a}}
\newcommand{\qvec}{\boldsymbol{q}}
\newcommand{\lc}{\ell_{\text{cut}}(\gras{r})}
\newcommand{\kc}{k_{\text{cut}}(\gras{r})}
\newcommand{\kF}{k_{F}(\gras{r})}
\newcommand{\Mstar}{M^{*}(\gras{r})}
\newcommand{\gras}[1]{\boldsymbol{#1}}
\newcommand{\tensor}[1]{\mathsf{#1}}
\newcommand{\capital}[1]{\mathscr{#1}}

\newcommand{\bnl}{\begin{eqnalpha}}
\newcommand{\enl}{\end{eqnalpha}}
\newcommand{\bnll}[1]{\begin{eqnalphalabel}{#1}}
\newcommand{\enll}{\end{eqnalphalabel}}

\newcommand{\bbox}[1]{\mbox{{\boldmath{$#1$}}}}
\newcommand{\cbox}[1]{\mbox{{\boldmath{${\scriptstyle#1}$}}}}
\newcommand{\svec}[1]{\bbox{#1}}
\newcommand{\ivec}[1]{\vec{#1}}

\newcommand{\reqrp}{\mbox{{\scriptsize{\boldmath{$r$=$r'$}}}}}

\newcommand{\keyw}{{\bf Keyword:}}
\newcommand{\key}[1]{\vspace{1ex}\noindent\keyw{\spc}{\tk{#1}}
                         \newline\phantom{\keyw{\spc}{\tk{#1}}}{\spc}}
\newcommand{\keywo}[1]{{keyword {\tk{#1}}}}
\newcommand{\keyspace}{\vspace{2ex}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bn}{\begin{eqnarray}}
\newcommand{\en}{\end{eqnarray}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}

\newcommand{\thalf}{{\textstyle{\frac{1}{2}}}}
\newcommand{\third}{{\textstyle{\frac{1}{3}}}}
\newcommand{\tquar}{{\textstyle{\frac{1}{4}}}}
\newcommand{\jde}{{{\cal J}^{(2)}}}
\newcommand{\jun}{{{\cal J}^{(1)}}}
\newcommand{\umi}{{$\hbar^2$/MeV}}
\newcommand{\ho}{{\hbar\omega}}
\newcommand{\hozero}{{\hbar\omega_0}}
\newcommand{\hoperp}{{\hbar\omega_\perp}}
\newcommand{\hox}{{\hbar\omega_x}}
\newcommand{\hoy}{{\hbar\omega_y}}
\newcommand{\hoz}{{\hbar\omega_z}}
\newcommand{\ph}{\phantom{$-$}}
\newcommand{\pg}{\phantom{-}}
\newcommand{\rmd}{{\rm d}}

\newcommand{\ti}[1]{#1\index{#1}}
\newcommand{\tii}[2]{#1\index{#1 #2}}
\newcommand{\tv}[1]{{\tt{#1}}\index{#1}}
\newcommand{\tk}[1]{{\tt{#1}}\index{#1}}
\newcommand{\ts}[1]{{\pr{#1}}\index{#1}}
\newcommand{\tf}[1]{{\tt{#1}}\index{#1}}
\renewcommand{\ti}[1]{#1}
\renewcommand{\tii}[2]{#1}
\renewcommand{\tv}[1]{\textcolor{red}    {{\tt{#1}}}}
\renewcommand{\tk}[1]{\textcolor{blue}   {{\tt{#1}}}}
\renewcommand{\ts}[1]{\textcolor{green}  {{\pr{#1}}}}
\renewcommand{\tf}[1]{\textcolor{magenta}{{\tt{#1}}}}
\renewcommand{\tv}[1]{{\tt{#1}}}
\renewcommand{\tk}[1]{{\tt{#1}}}
\renewcommand{\ts}[1]{{\pr{#1}}}
\renewcommand{\tf}[1]{{\tt{#1}}}

\hyphenation{mo-no-pole quad-ru-pole oc-tu-pole su-per-de-for-med}
\hyphenation{qua-dra-ture}

%
%  REDEFINITION OF COMMANDS
%
\renewcommand{\topfraction}{1.0}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\floatpagefraction}{1.0}

\newenvironment{eqnalpha}{\setcounter{leteq}{1}
\renewcommand{\theequation}{\arabic{equation}\alph{leteq}}
\begin{eqnarray}}{\end{eqnarray}%
\renewcommand{\theequation}{\arabic{equation}}}

\newenvironment{eqnalphalabel}[1]{\setcounter{leteq}{1}
\raisebox{0cm}[0cm][0cm]{\begin{minipage}{1cm}%
\begin{eqnarray}\label{#1}&&\nonumber\end{eqnarray}\end{minipage}}
\renewcommand{\theequation}{\arabic{equation}\alph{leteq}}
\begin{eqnarray}}{\end{eqnarray}%
\renewcommand{\theequation}{\arabic{equation}}}

